Relieving the Wireless Infrastructure: When Opportunistic Networks Meet Guaranteed Delays

Major wireless operators are nowadays facing network capacity issues in striving to meet the growing demands of mobile users. At the same time, 3G-enabled devices increasingly benefit from ad hoc radio connectivity (e.g., Wi-Fi). In this context of hybrid connectivity, we propose Push-and-track, a content dissemination framework that harnesses ad hoc communication opportunities to minimize the load on the wireless infrastructure while guaranteeing tight delivery delays. It achieves this through a control loop that collects user-sent acknowledgements to determine if new copies need to be reinjected into the network through the 3G interface. Push-and-Track includes multiple strategies to determine how many copies of the content should be injected, when, and to whom. The short delay-tolerance of common content, such as news or road traffic updates, make them suitable for such a system. Based on a realistic large-scale vehicular dataset from the city of Bologna composed of more than 10,000 vehicles, we demonstrate that Push-and-Track consistently meets its delivery objectives while reducing the use of the 3G network by over 90%.

==> real-case.tex <==
\section{Datasets and Preliminary Analysis}
\label{sec:real-case}

%
We evaluate the proposed dissemination algorithm on a large-scale vehicular mobility excerpt of a city-wide dataset of the municipality of Bologna (Italy).
elaborated during the iTetris project~\cite{itetris}.
We specifically focus on a urban subset of the municipality of Bologna's road network: the so-called \emph{Ringway}. The Ringway section covers $20.6 km^2$, includes $191 km$ of roads and exhibits diversity in terms of road types: a ring-shaped main road yields to various entry points to the historical city center.

%
We select the SUMO (Simulation of Urban MObility) platform to simulate the Ringway traffic conditions with a large number of vehicles.
%
SUMO~\cite{sumo} is an open-source microscopic vehicular movement simulator developed by the Centre for Applied Informatics and the Institute of Transport Research at the German Aerospace Centre. The project started in 2001 with the goal of supporting the vehicular research community with a common platform to test and compare models of vehicle behavior, traffic light optimization, and vehicle routing.
%
To model individual vehicle movement, SUMO uses a space-continuous and time-discrete car-following model developed by Stefan Krauss~\cite{krauss}. 
The mobility model features a collision-free movement simulation constrained by the multi-lane road network as well as by the traffic light control system, lane changing rules and junction-based right-of-way rules.   

%
%
The prerequisite data for performing a SUMO microscopic traffic simulation includes an accurate model of the road network and intersections, the profile of vehicles and their assigned routes. To obtain a relevant dataset, we use traffic conditions measurements realized by the municipality of Bologna (Italy) on their road network.
The supplied raw data includes measurements of circulating vehicles acquired by XX induction loops spread over the city and a synthesis of user surveys on usual trips within the city. Using this raw data, the OD (Origin-Destination) vehicle flow matrices give us a macroscopic view of the scenario under consideration. The traffic demands are then mapped onto the highly-accurate Bologna road network with individual vehicle route assignments.
The macroscopic traffic demands on the city road network are extracted from measurements during common weekday peak hours (from 8 am to 9 am), ignoring Monday and Friday to avoid exotic traffic patterns due to the week-end proximity. 
For sake of clarity, we don't detail the derivation of the microscopic route assignments from the macroscopic traffic demands any further in this paper, and we assert that the mobility traces are representative of the aforementioned traffic conditions.


%
We assume that all the vehicles may communicate using the IEEE 802.11p (DRAFT??) standard~\cite{80211p}. The standard operates in the XX frequency range and defines XX channels with a 10MHz bandwidth. It offers a range of transmission rates from 3Mb/s to 27Mb/s. \todo{maybe a little bit more on vehicular wifi as it is the only place we will mention it}.
As wireless propagation models are not the core of this paper, we assume a deterministic model where a packet is successfully received if the receiver's distance is below a certain indicative value. Following a pragmatic approach, we consider DSRC path loss model approximations and measurement in a urban line-of-sight environment performed by Cheng et al.~\cite{cheng2007mobile} 
The path-loss may be accurately approximated by a dual-slope piecewise-linear model with a breakpoint at distance $d=100m$. Considering a typical receive power threshold at -95 dBm, the model approximation and pathloss measurements with the DSRC prototypes corroborate our assumption of a successful packet reception at an indicative critical distance $d=100m$.
%
%
We design our dissemination algorithm for non-safety applications, which have released constraints on delivery time. This may include traffic information or software update distribution. Considering the profile of target applications, we assume their operation on a Service Channel (SCH) with a transmission bitrate at 6Mb/s, which is appropriate for short-range robust communications.
%

%


%
\subsection{Dataset analysis}
For highlighting the potential communications between the vehicles, we designed a custom simulator which runs the mobility traces with the chosen deterministic propagation model and transmission bitrate.
%
%
We analyse thereafter the vehicular traffic and network connectivity statistics of the simulation. After a warm-up period, the traffic is simulated during 3600s, which leads to a total number of XX22,000 simulated vehicles with an average of XX3000 vehicles simultaneously.

The average amount of traffic and on the different road segments are depicted in Figure~\cite{fig_map}. It exposes a relatively larger amount of traffic on the surrounding ring-shaped road than on the capillary network with traffic jams occuring on intersections.
%
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{entered_speed_color}
\caption{Anamorphic representation of simulated Bologna ringway road network. The number of vehicles on a given road is represented by its thickness using a logarithmic scale. The vehicle speed on a road is represented by the color. Both values are averaged over the simulation duration.}
\label{fig_map}
\end{figure}

The travel times CDF is depicted in Figure~\ref{fig_travel_times}.
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{transit_times_cdf_1h}
\caption{Travel times CDF}
\label{fig_travel_times}
\end{figure}

The contacts CDF is depicted in Figure~\ref{fig_contacts_cdf_1h}.
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{contacts_cdf_1h}
\caption{Contacts CDF}
\label{fig_contacts_cdf_1h}
\end{figure}

The number of connected components over time is depicted in Figure~\ref{fig_components}
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{components}
\caption{Number of connected components}
\label{fig_components}
\end{figure}

%

%


